Avengers Ensemble! Improving Transferability of Authorship Obfuscation

Stylometric approaches have been shown to be quite effective for real-world authorship attribution. To mitigate the privacy threat posed by authorship attribution, researchers have proposed automated authorship obfuscation approaches that aim to conceal the stylometric artefacts that give away the identity of an anonymous document's author. Recent work has focused on authorship obfuscation approaches that rely on black-box access to an attribution classifier to evade attribution while preserving semantics. However, to be useful under a realistic threat model, it is important that these obfuscation approaches work well even when the adversary's attribution classifier is different from the one used internally by the obfuscator. Unfortunately, existing authorship obfuscation approaches do not transfer well to unseen attribution classifiers. In this paper, we propose an ensemble-based approach for transferable authorship obfuscation. Our experiments show that if an obfuscator can evade an ensemble attribution classifier, which is based on multiple base attribution classifiers, it is more likely to transfer to different attribution classifiers. Our analysis shows that ensemble-based authorship obfuscation achieves better transferability because it combines the knowledge from each of the base attribution classifiers by essentially averaging their decision boundaries.

==> tables/tbl-attack-success-rate.tex <==
\begin{table}[ht]
\begin{tabular}{llr}
\toprule
Classifier & Attack Success Rate \\
\midrule
writeprintsRFC &  0.215278 \\
writeprintsSVM &  0.256944 \\
writeprintsEnsemble &  0.267857 \\
\bottomrule
\end{tabular}
\caption{Attack success rate of the different classifiers.}
\label{tbl:attack-success-rate}
\end{table}

